Light on the Infinite Group Relaxation

This is a survey on the infinite group problem, an infinite-dimensional relaxation of integer linear optimization problems introduced by Ralph Gomory and Ellis Johnson in their groundbreaking papers titled "Some continuous functions related to corner polyhedra I, II" [Math. Programming 3 (1972), 23-85, 359-389]. The survey presents the infinite group problem in the modern context of cut generating functions. It focuses on the recent developments, such as algorithms for testing extremality and breakthroughs for the k-row problem for general k >= 1 that extend previous work on the single-row and two-row problems. The survey also includes some previously unpublished results; among other things, it unveils piecewise linear extreme functions with more than four different slopes. An interactive companion program, implemented in the open-source computer algebra package Sage, provides an updated compendium of known extreme functions.

==> Makefile <==
LATEX=latex
PDFLATEX=pdflatex
FIG2DEV=fig2dev
BIBTEX=bibtex

FIGURESDIRPREFIX=

MAINTEXFILE=igp-survey

all: $(MAINTEXFILE).pdf

%.pstex_t: %.fig #Makefile
	$(FIG2DEV) -L pstex_t -p $*.pstex $< $@

%.pstex: %.fig #Makefile
	$(FIG2DEV) -L pstex $< $@

%.pdftex_t: %.fig #Makefile
	$(FIG2DEV) -L pdftex_t -p $*.pdf $< $@

%.pdf: %.fig #Makefile
	$(FIG2DEV) -L pdftex $< $@

SURVEY_GRAPHICS_SOURCES=			\
	figureProjection.fig			\
	figureKKMcircleSmallerAdjust.fig

SURVEY_GENERATED_GRAPHICS=$(SURVEY_GRAPHICS_SOURCES:%.fig=$(FIGURESDIRPREFIX)%.pdftex_t) $(SURVEY_GRAPHICS_SOURCES:%.fig=$(FIGURESDIRPREFIX)%.pdf) 

#$(SURVEY_GRAPHICS_SOURCES:%.fig=%.pstex_t) $(SURVEY_GRAPHICS_SOURCES:%.fig=%.pstex)

SURVEY_SOURCES=Makefile $(MAINTEXFILE).tex $(SURVEY_GRAPHICS_SOURCES:%.fig=$(FIGURESDIRPREFIX)%.fig) \
	sage-commands.tex function-poset.tex compendium.tex notation.tex \
	2d-perturbation-IPCOext-version-as-submitted.aux 

SURVEY_STYLES = equipert.sty

SURVEY_GRAPHICS=$(SURVEY_GENERATED_GRAPHICS)						\
	automorphism-from.pdf								\
	automorphism-to.pdf								\
	bccz_counterexample.pdf								\
	bccz_counterexample_with_ticks-0.pdf						\
	bccz_counterexample_with_ticks-1.pdf						\
	bccz_counterexample_with_ticks-2.pdf						\
	bccz_counterexample_with_ticks-3.pdf						\
	bccz_counterexample_with_ticks.pdf						\
	bhk_irrational-2d_diagram.pdf							\
	bhk_irrational.pdf								\
	bhk_irrational_extreme_limit_to_rational_nonextreme-2d_diagram.pdf		\
	bhk_irrational_extreme_limit_to_rational_nonextreme-completion.pdf		\
	bhk_irrational_extreme_limit_to_rational_nonextreme-covered_intervals.pdf	\
	bhk_irrational_extreme_limit_to_rational_nonextreme-moves.pdf			\
	bhk_irrational_extreme_limit_to_rational_nonextreme-perturbation-1.pdf		\
	bhk_irrational_extreme_limit_to_rational_nonextreme_1-2d_diagram.pdf		\
	bhk_irrational_extreme_limit_to_rational_nonextreme_1-completion.pdf		\
	bhk_irrational_extreme_limit_to_rational_nonextreme_1-covered_intervals.pdf	\
	bhk_irrational_extreme_limit_to_rational_nonextreme_2-2d_diagram.pdf		\
	bhk_irrational_extreme_limit_to_rational_nonextreme_2-completion.pdf		\
	bhk_irrational_extreme_limit_to_rational_nonextreme_2-covered_intervals.pdf	\
	chen_4_slope.pdf								\
	dg_2_step_mir.pdf								\
	dg_2_step_mir_limit.pdf								\
	dr_projected_sequential_merge_3_slope.pdf					\
	drlm_2_slope_limit.pdf								\
	drlm_2_slope_limit_1_1.pdf							\
	drlm_3_slope_limit.pdf								\
	drlm_backward_3_slope.pdf							\
	drlm_gj_2_slope_extreme_limit_to_nonextreme-2d_diagram.pdf			\
	drlm_gj_2_slope_extreme_limit_to_nonextreme-covered_intervals.pdf		\
	drlm_gj_2_slope_extreme_limit_to_nonextreme-perturbation-1.pdf			\
	drlm_gj_2_slope_extreme_limit_to_nonextreme_3-2d_diagram.pdf			\
	drlm_gj_2_slope_extreme_limit_to_nonextreme_3-covered_intervals.pdf		\
	drlm_gj_2_slope_extreme_limit_to_nonextreme_50-2d_diagram.pdf			\
	drlm_gj_2_slope_extreme_limit_to_nonextreme_50-covered_intervals.pdf		\
	drlm_not_extreme_1-2d_diagram.pdf						\
	drlm_not_extreme_1-completion.pdf						\
	drlm_not_extreme_1-covered_intervals.pdf					\
	drlm_not_extreme_1-moves.pdf							\
	drlm_not_extreme_1-perturbation-1.pdf						\
	drlm_not_extreme_1-restricted-1-2d_diagram.pdf					\
	drlm_not_extreme_1-restricted-1.pdf						\
	drlm_not_extreme_1-restricted-4-2d_diagram.pdf					\
	drlm_not_extreme_1-restricted-4-perturbation-1.pdf				\
	drlm_not_extreme_1-restricted-4-perturbation-2.pdf				\
	drlm_not_extreme_1-restricted-4-perturbation-3.pdf				\
	drlm_not_extreme_1-restricted-4.pdf						\
	figureKKM.pdf									\
	figureKKMcircle.pdf								\
	figureKKMcircleSmallerAdjust.pdf						\
	figureKKMnoSquare.pdf								\
	figureKKMnoSquare2.pdf								\
	figurePositivePhi.pdf								\
	figureProjection.pdf								\
	figureReflectionPoints.pdf							\
	figure_interval_lemma_1.pdf							\
	figure_interval_lemma_2.pdf							\
	figure_interval_lemma_3.pdf							\
	flatFunction.pdf								\
	flatFunction3and4.pdf								\
	fourSlope1.pdf									\
	gj_2_slope-2d_complex.pdf							\
	gj_2_slope-2d_diagram.pdf							\
	gj_2_slope.pdf									\
	gj_2_slope_repeat.pdf								\
	gj_forward_3_slope-2d_diagram.pdf						\
	gj_forward_3_slope.pdf								\
	gmic.pdf									\
	graph-0.pdf									\
	graph-1.pdf									\
	graph-12.pdf									\
	graph-123.pdf									\
	graph-13.pdf									\
	graph-2.pdf									\
	graph-23.pdf									\
	graph-3.pdf									\
	graph-b.pdf									\
	hierarchy.pdf									\
	hildebrand_2_sided_discont_1_slope_1.pdf					\
	hildebrand_2_sided_discont_2_slope_1.pdf					\
	hildebrand_5_slope_22_1.pdf							\
	hildebrand_5_slope_24_1.pdf							\
	hildebrand_5_slope_28_1.pdf							\
	hildebrand_discont_3_slope_1.pdf						\
	interpolate_to_infinite_group-from.pdf						\
	interpolate_to_infinite_group-to.pdf						\
	kf_n_step_mir.pdf								\
	kzh_7_slope_1.pdf								\
	kzh_28_slope_1.pdf								\
	ll_strong_fractional.pdf							\
	multiplicative_homomorphism-from.pdf						\
	multiplicative_homomorphism-to.pdf						\
	not_extreme_1-2d_diagram.pdf							\
	not_extreme_1-covered_intervals.pdf						\
	not_extreme_1-perturbation-1.pdf						\
	not_extreme_1-perturbation-2.pdf						\
	not_minimal_2-2d_diagram.pdf							\
	polyhedralComplex2.pdf								\
	projected_sequential_merge-from.pdf						\
	projected_sequential_merge-to.pdf						\
	publication_diag_colors.pdf							\
	publication_diag_constrained_6.pdf						\
	restrict_to_finite_group-from.pdf						\
	restrict_to_finite_group-to.pdf							\
	restrict_to_finite_group_3-from.pdf						\
	restrict_to_finite_group_3-to.pdf						\
	rlm_dpl1_extreme_3a.pdf								\
	threeSlopeGomoryJohnson.pdf							\
	twoSlope1.pdf									\
	twoSlope2.pdf									\
	two_slope_fill_in-from.pdf							\
	two_slope_fill_in-to.pdf


BIB=../bib/MLFCB_bib.bib

.PHONY: figures

figures: $(SURVEY_GRAPHICS) 

$(MAINTEXFILE).pdf: $(MAINTEXFILE).tex $(SURVEY_GRAPHICS) $(BIB)
	$(PDFLATEX) -halt-on-error "$<"
	$(BIBTEX) $(MAINTEXFILE)
	$(PDFLATEX) -halt-on-error "$<"
	$(PDFLATEX) -halt-on-error "$<"

SURVEY_SOURCES_AND_MORE=$(SURVEY_SOURCES) $(SURVEY_GRAPHICS) $(SURVEY_STYLES)

.PHONY: arxiv
arxiv:
	COPYFILE_DISABLE=true tar -cf $(CURDIR)/$(MAINTEXFILE).tar	\
		$(MAINTEXFILE).bbl					\
		$(SURVEY_SOURCES)					\
		$(SURVEY_GRAPHICS)					\
		$(SURVEY_STYLES)
	rm -f $(MAINTEXFILE).tar.gz
	gzip $(MAINTEXFILE).tar

clean: 
	-rm -f *.bak *.aux *.log *.bbl *.blg $(SURVEY_GENERATED_GRAPHICS)


